Causal Understanding For Video Question Answering

Video Question Answering is a challenging task, which requires the model to reason over multiple frames and understand the interaction between different objects to answer questions based on the context provided within the video, especially in datasets like NExT-QA (Xiao et al., 2021a) which emphasize on causal and temporal questions. Previous approaches leverage either sub-sampled information or causal intervention techniques along with complete video features to tackle the NExT-QA task. In this work we elicit the limitations of these approaches and propose solutions along four novel directions of improvements on theNExT-QA dataset. Our approaches attempts to compensate for the shortcomings in the previous works by systematically attacking each of these problems by smartly sampling frames, explicitly encoding actions and creating interventions that challenge the understanding of the model. Overall, for both single-frame (+6.3%) and complete-video (+1.1%) based approaches, we obtain the state-of-the-art results on NExT-QA dataset.

==> sections/related_work/ds_bias_related_work.tex <==
% Biases can originate from two main sources; the model and the dataset. The former can arise from a multitude of situations starting from something as simple as class imbalance, to correlations between different categories in the prediction and attributes within the dataset, and could also be due to systemic social biases present in the dataset. The latter is due to the fact that it can make the model too dependent on a single training signal, which will make it ignore others. For example, a CNN will pay more attention to the textures, rather than the objects within the image. 

% Dataset bias can be further subdivided on the basis of whether it arises due to spurious correlations in the dataset or due to systematic biases present in the dataset. A common example of the former is shortcut bias in which a certain correlation, can cause the model to learn relationships that hurt generalization \cite{geirhos2020shortcut}. A particularly insidious example of the latter is Fairness bias, in which the model propagates the stereotypes present in the data into its predictions.

% \cite{AgarwalBehaviorVQA} and \cite{JabariVQA} explore how much the model truly understands the modalities for the VQA dataset \cite{VQA}. By just capturing some parts of the question and not really even relying on the whole image, the models are able to map certain question words to certain answers.
% They observe, that it does not make use of the full information used in the question, nor does it really make use of the whole image. In fact, just by capturing some parts of the question, it is able to answer the question just by understanding the certain question words can be directly mapped to certain answers. 
% \cite{GururanganAnnotationArtifacts,GevaModelAnnotator} do a systematic study into biases present in text modality wherein answering questions is possible by relying on small part of the context and/or exploiting annotator bias.
% It is possible to answer questions by just looking a small part of the context or by exploiting the presence of annotator bias. 
% \cite{BirhaneMisogeny} show the danger of using a model to curate dataset, as the biases in the model get transferred to the dataset. \cite{geirhos2020shortcut} and \cite{Ye_Kovashka_2021} describe learning shortcuts' behaviour in the case of deep neural networks. 

% Works such as \cite{BrasAFL, GatPerceptualScore,ChoDallEval} propose methods to evaluate biases in models. The first method uses dataset pruning to get rid of very similar examples, while retaining the overall diversity within the dataset. The second method isolated effect of each modality, so that it can attribute the performance gain by adding the missing modality. The third method makes use of systematic tests to decide the correctness of text to image generative models such as DALLE-E \cite{DaLLe}.

% Finally,  \cite{GANDebiasing} uses the latents within Progressive GAN \cite{progGAN} to generate images that removes biases within the dataset. \cite{xu2018fairgan} tries to generate images by using a loss term that targets bias in the generated image.

\subsection{Dataset Biases}
Significant research on leveraging different dataset biases for performing downstream tasks. Partial usage of question while not relying on the image\cite{AgarwalBehaviorVQA,JabariVQA}, exploiting annotator biases\cite{GururanganAnnotationArtifacts, GevaModelAnnotator}, using biases from models for dataset curation\cite{BirhaneMisogeny}, learning shortcut behaviours from training the neural networks\cite{geirhos2020shortcut, Ye_Kovashka_2021}.
Works such as \cite{BrasAFL, GatPerceptualScore,ChoDallEval} propose methods such as dataset pruning to eliminate similar examples, use systematic tests to decide the correctness of text-to-image generative models such as DALLE \cite{DaLLe}.\cite{GANDebiasing} uses latent within Progressive GAN \cite{progGAN} to generate images that remove biases within the dataset. \cite{xu2018fairgan} generate images which utilize the loss term that targets bias in generated image.
